Streaming k-Means Clustering with Fast Queries

We present methods for k-means clustering on a stream with a focus on providing fast responses to clustering queries. Compared to the current state-of-the-art, our methods provide substantial improvement in the query time for cluster centers while retaining the desirable properties of provably small approximation error and low space usage. Our algorithms rely on a novel idea of "coreset caching" that systematically reuses coresets (summaries of data) computed for recent queries in answering the current clustering query. We present both theoretical analysis and detailed experiments demonstrating their correctness and efficiency

==> algorithm-etc.tex <==

\remove{
The main idea in coreset caching is the following.

%---------------------------------------------
\subsection{Algorithm Description}
\label{sec:algorithm}
%---------------------------------------------
{\color{red} What is $\beta$, max buckets per level, $m$ size of a coreset.\\}


We describe our algorithm for streaming $k$-means clustering. The basic data structure is a ``bucket'' $b$ which is a 4-tuple $(C,l,r,\ell)$, with the following invariant: $C$ is a level $\ell$ coreset of substream $S(l,r)$. Thus each bucket consists of a coreset of a substream of $S$. For bucket $b = (C,l,r,\ell)$, let $C(b)$ denote the coreset in $b$, $\leftep(b)=l$ the left endpoint of $b$, $\rightep(b)=r$ the right endpoint of $b$, and $\level(b) = \ell$ the level of the coreset $C(b)$. The span of the bucket $b$, denoted by $\bspan(b)$, is defined as the interval $[\leftep(b), \rightep(b)]$.\\

The algorithm maintains a data structure $Q$ that consists of sets of buckets $Q_{\ell}$  at different levels $\ell=0,1,2,\ldots$. This data structure has the following invariants. Each bucket $b \in Q_j$ is a level $j$ coreset of a substream of $S$.

A container of coresets $T$ (such as $Q$ and $\cache$) provides the following operation: $\lookup(T, l,r)$, defined as follows. If there is a bucket $b = (C,l,r,\ell)$ within $T$, then return $b$.  Otherwise, return $\emptyset$.

%-------------------
\begin{itemize}
\item
The spans of different buckets in $Q$ are disjoint.

\item
For each $\ell \ge 0$, the number of buckets in $Q_{\ell}$ cannot exceed $\beta$.

\item
For each $\ell > 0$, the union of the span of all buckets in $Q_{\ell}$ is a single continuous interval.

\item
The union of the spans of all buckets in $Q$ equals the interval $[1,t]$.
\end{itemize}
%---------------

The algorithm also maintains an additional structure, a set of buckets, $\cache$ that we call the ``coreset-cache''.  {\color{red} Say more about the cache.}

\remove{
%---------------------------------------------
\begin{definition}[Major and Minor]
\label{defn:maj-min}
For positive integer $n > 0$, consider the unique decomposition of $n$ into a sum of powers of $2$: 
$n = \sum_{i=0}^j2^{\alpha_i}$, where $\alpha_j>\alpha_{j-1}>\cdots>\alpha_0\geq 0$.  
Let $\minor(n) = 2^{\alpha_0}$, the smallest term in the decomposition. Let $\major(n) = n - \minor(n)$. Note that when $n$ is a power of $2$, $\major(n) = 0$.
\end{definition}
%---------------------------------------------
}

%---------------------
\begin{algorithm}
\label{algo:fkm-init}
\DontPrintSemicolon
\caption{Initialization: Initialize Data Structures}
$Q \gets \emptyset$\;
$\cache \gets \emptyset$\;
\end{algorithm}
%------------------

%---------------------
\begin{algorithm}
\label{algo:fkm-process}
\DontPrintSemicolon
\caption{Update($B_n$): Update Data structures at Timestep $n$.}
\KwIn{Batch $B_n$}
\KwOut{$k$-means cluster centers of $S(n)$}

Add bucket $(B_n, n, n, 0)$ to $Q$\;

$j \leftarrow 0$\;

\While{$|Q_j| \ge r$}
{
  $b_1 \gets \bunion(Q_j)$ \;
  $b_2 \gets (\coreset\left(k, \eps, C(b_1) \right), \leftep(b_1), \rightep(b_1), 1+ \level(b_1))$\;
  Add bucket $b_2$ to $Q_{j+1}$ \;
  Set $Q_j$ to $\emptyset$\; 
  $j \gets (j+1)$ \;
}


$n_1 \gets \major(n)$ and $n_2 \gets \minor(n)$\;
Let $n_2=\beta r^{\alpha}$, where $\alpha, \beta\in Z^+$ and $\beta<r$ \;

$l \gets n_1+1$ \;
$a \gets \emptyset$ \;

\For{$i=1$ \emph{\KwTo} $\beta$}
{
	$a \gets a \cup \lookup(Q, l, l+r^{\alpha}-1)$ \;
	$l \gets l+r^{\alpha}$\;
} 


\eIf {$n_1$ is $0$}
{
	$C_n \gets a$\;
}
{
	$b \gets \lookup(\cache, 1, n_1)$ \;
	$C_n \gets \coreset(k, \eps, a \cup b)$\;
}

\If{$n$ is divisible by $r$} 
{
From $\cache$, remove all buckets $b'$  such that $\rightep(b') \notin \partsum(n)$\;

Add $\left(C_n, 1, n, 1 + \max\{\level(a), \level(b)\} \right)$ to $\cache$\;
}

\Return $\kmpp(k, a \cup b)$\;
\end{algorithm}
%---------------------


%---------------------------------------------------------
\subsection{Correctness Proof and Analysis}
%---------------------------------------------------------

%---------------------------------------------------------
With the level of a coreset is known, the coreset approximation factor can be derived by the following lemma: \\
\begin{lemma}
\label{lemma:level-accuracy}
For a point set $P$ and integer $\ell \ge 0$, if $C = \coreset(k, \eps, \ell, P)$, then $C = \coreset(k, \eps', P)$ where $\eps' = \left(1+\eps \right)^{\ell} - 1$.
%For $i=0 \ldots \ell$, we have $C_i = \coreset(k, (1+epsilon)^\ell_i-1, \ell_i)$.
\end{lemma}

\begin{proof}
Let ${\cal P}(\ell)$ be the proposition: For any point set $P$, if $C = \coreset(k, \eps, \ell, P)$, then $C = \coreset(k, \eps', P)$ where $\eps' = \left(1+\eps \right)^{\ell} - 1$. We prove this lemma by induction on $\ell$. For the base case, consider $\ell=0$. By definition, $\coreset(k,\eps, 0, P) = P$, and $\coreset(k, 0, P) = P$, proving the base case.\\

Consider integer $L > 0$. Suppose that for each positive integer $\ell < L$,  ${\cal P}(\ell)$ was true. The task is to prove ${\cal P}(L)$. Suppose $C = \coreset(k, \eps, L, P)$. Then there must be an arbitrary partition of $P$ into sets $P_1, P_2, \ldots, P_q$ such that $\cup_{i=1}^q P_i = P$. For $i=1\ldots q$, let $C_i = \coreset(k, \eps, \ell_i, P_i)$ for $\ell_i < L$. Then $C$ must be of the form $\coreset(k, \eps, \cup_{i=1}^q C_i)$. \\

By the inductive hypothesis, it must be true that $C_i=\coreset(k, \eps_i, P_i)$ where $\eps_i = \left(1+\eps \right)^{\ell_i} - 1$. By the definition of a coreset and using $\ell_i \le (L-1)$, it is also true that $C_i = \coreset(k, \eps'', P_i)$ where $\eps'' = \left(1+\eps \right)^{(L-1)} - 1$.  Let $C' = \cup_{i=1}^q C_i$.  From Observation~\ref{obs:coreset1}, and using $P = \cup_{i=1}^q P_i$, it must be true that $C'= \coreset(k, \eps'', P)$. Since $C=\coreset(k,\eps,C')$ and using Observation~\ref{obs:coreset2}, we get  $C=\coreset(k, \gamma, P)$ where $\gamma=(1+\eps)(1+\eps'')-1$. Simplifying, we get $\gamma=(1+\eps)(1+ \left(1+\eps \right)^{(L-1)} - 1)-1 = \left(1+\eps \right )^L - 1$. This proves the inductive case ${\cal P}(L)$, completing the proof of the lemma.
\end{proof}
%---------------------------------------------------------

%-------------------
\begin{lemma}
\label{lemma:maxlevel at coreset-tree}
For each timestep $n$, the coreset in the coreset tree $Q$ is at maximum level $\left\lfloor \log n/\log r \right\rfloor$ where $r$ is the merge degree of $Q$.
\end{lemma}
%-------------------
\begin{proof}
We first note that for any level $\ell \ge 0$, there are no more than $r$ buckets at level $\ell$ within $Q$; if there were more than $r$ buckets, they will be merged into a single bucket at level $\ell+1$. Next, in order to get a single bucket at level $\ell$, it is necessary to merge $r$ buckets at level $(\ell-1)$, $r^2$ buckets at level $(\ell-2)$, and so on. So for a single bucket at level $\ell$, it requires $r^{\ell}$ level $0$ buckets to merge. Suppose $\ell_{max}$ is the maximum level of a bucket within $Q$. Since the coreset tree has $n$ level $0$ buckets received, it must be true that $r^{\ell_{max}} \le n$, which leads to $\ell_{max} = \left\lfloor \log n/\log r \right\rfloor$.
\end{proof}
%-------------------

%-------------------
\begin{figure*}
  \centering
  \includegraphics[width=0.4\textwidth]{./figures/tree.jpg}
  \caption{coreset merge from coreset tree and cache (timestep=$368$, merge degree $r=5$), 
  inside each node shows the left to right endpoint batch of the bucket, 
  above each node shows the number in $5$-nary format}
  \label{fig:coreset merge}
\end{figure*}
%-------------------

%-------------------
\begin{lemma}
\label{lemma:maxlevel at cache}
At the end of each timestep $n$, the coreset in the $\cache$ is at maximum level $2 \cdot \left\lfloor \log n/\log r \right\rfloor$.
\end{lemma}
%---------------------------------------------------------

\begin{proof}
Let us expand $n$ as an $r$-ary number.

Refer to the process of Algorithm~\ref{algo:fkm-process}, if $\major(n)$ is $0$, the new coreset $C_n$ is directly constructed by a copy of the coreset in $Q$. Based on the Lemma~\ref{lemma:maxlevel at coreset-tree}, the new coreset is at maximum level $\left\lfloor \log n/\log r \right\rfloor$. \\

When $\major(n)$ is not $0$, consider $n$ in $r$ radix base format: $n=\sum_{i=0}^j\beta_ir^{\alpha_i}$, where $\alpha_j>\alpha_{j-1}>\cdots>\alpha_0\ge 0$. Algorithm~\ref{algo:fkm-process} constructs coreset $C_n$ by merging a bucket $b_{cache}$ from $\cache$ which contains the coreset of batches $\left[ 1, \sum_{i=1}^j\beta_ir^{\alpha_i} \right]$, and another bucket $b_Q$ from the coreset tree $Q$ which contains the coreset of batches $\left[ 1+\sum_{i=1}^j\beta_ir^{\alpha_i}, n \right]$. 
See Figure~\ref{fig:coreset merge} as an example, which shows the history of constructing the new coreset $C_n$ at timestep $368$. For each internal node of the merge tree, the left child is the bucket from the $\cache$ and the right child is the bucket from coreset tree.  
The left most child contains the coreset of batches $\left[1, \beta_jr^{\alpha_j}\right]$ which is at level $\alpha_j$. Starting from the left most child, as each merge increments the coreset level by $1$ and the total number of merges equals $j$, we can derive the level of coreset $C_n$ by $\left(j+\alpha_j\right)$. With $j \le \alpha_j \le \left\lfloor \log n/\log r \right\rfloor$, the level of coreset $C_n$ at maximum level $2 \cdot \left\lfloor \log n/\log r \right\rfloor$. \\

So at each timestep $n$, the new coreset stored in the $\cache$ is at at maximum level $2 \cdot \left\lfloor \log n/\log r \right\rfloor$, which leads to all the coresets in the $\cache$ is at maximum level $2 \cdot \left\lfloor \log n/\log r \right\rfloor$.
\end{proof}
%---------------------------------------------------------


\begin{lemma}
\label{lemma:final accuracy}
At the end of each time step $n$, if $\eps=\tilde{c}\cdot\frac{\log r}{2\log n}$ for some constant $\tilde{c}<\ln 2$, 
then Algorithm~\ref{algo:fkm-process} returns a set of $k$ centers $C$ such that 
$E\left[\phi_C(S(n))\right] \le 16(\ln k+2) \cdot \phi_{OPT}(S(n))$.
\end{lemma}
%-------------------
\begin{proof}
At time step $n$, based on the Lemma~\ref{lemma:maxlevel at cache}, the coreset $C_n$ is at level no greater than 
$2 \left\lfloor\log n/\log r \right\rfloor$. 
So using Lemma~\ref{lemma:level-accuracy}, $C_n$ is an $\eps'$-coreset for $S(n)$ where 

\[ \begin{split} 
\eps' &= \left[ \left(1 + \tilde{c}\cdot\frac{\log r}{2\log n}\right)^{\frac{2\log n}{\log r}}-1 \right] \\
&\le \left[ e^{\left(\tilde{c}\cdot \frac{\log r}{2\log n}\right)\cdot \frac{2\log n}{\log r}}-1 \right] = e^{\tilde{c}}-1 < 1
\end{split} 
\]

$S(n)$ is the received point set till time step $n$ and we define $O1$ is the set of $k$ centers which achieves optimal $\km$ clustering cost for $S(n)$. From the definition of coreset, 
\begin{equation}
\label{eq:final accuracy eq1}
\phi_{O1}(C_n) \le (1+\eps')\phi_{O1}(S(n)) \le 2\phi_{O1}(S(n))
\end{equation}
\\

Let $O2$ be the set of $k$ centers which achieves optimal $\km$ clustering cost for $C_n$. $C$ is the final $k$ centers generated by running $\kmpp$ $C_n$. Using Theorem~\ref{theo:kmeans++} and using $\phi_{O2}(C_n) \le \phi_{O1}(C_n)$, we have 
\begin{equation}
\label{eq:final accuracy eq2}
E\left[ \phi_C(C_n) \right] \le 8(\ln k+2)\cdot\phi_{O2}(C_n) \le 8(\ln k+2)\cdot\phi_{O1}(C_n)
\end{equation}
Using Equation~\ref{eq:final accuracy eq1} and \ref{eq:final accuracy eq2} we get $E\left[ \phi_C(C_n) \right] \le 16(\ln k+2)\cdot\phi_{O1}(S(n))$.
\end{proof}
%-------------------


\begin{lemma}
The space complexity of Algorithm~\ref{algo:fkm-process} is $O\left(\frac{kdr\log^7n}{\log^7r}\right)$ words. 
\end{lemma}
%-------------------
\begin{proof}
Using the Theorem~\ref{theo:coreset build}, the capacity of a bucket $m=O\left(\frac{kd}{\eps^6}\right)$. Based on Lemma~\ref{lemma:final accuracy}, we have set $\eps=\tilde{c}\cdot\frac{\log r}{2\log n}$ where $\tilde{c}$ is a constant. So the bucket size $m$ is $O\left(\frac{kd\log^6n}{\log^6r}\right)$. 
At each time step $n$, from Lemma~\ref{lemma:maxlevel at coreset-tree} the maximum level of a coreset in the coreset tree is $\left\lfloor\log n/\log r\right\rfloor$ and each level has no more than $r$ buckets, so the coreset tree $Q$ has $O\left(\frac{r \log n}{\log r}\right)$ buckets. The space complexity of $Q$ is $O\left(\frac{m r \log n}{\log r}\right)$ words.
For the space complexity of the $\cache$, consider at the end of each time step, we only keep the bucket $b'$ such that $\rightep(b') \in \partsum(n)$. 
As the number of partsums of a number $n$ is $\left\lceil \log n/\log r \right\rceil$, the number of buckets in the $\cache$ is always $O\left(\log n/\log r \right)$. So the space complexity of the $\cache$ is $O\left(\frac{m \log n}{\log r}\right)$ words.
Thus, the total space complexity of Algorithm~\ref{algo:fkm-process} is $O\left(\frac{kdr\log^7n}{\log^7r}\right)$.
\end{proof}
%-------------------


%-------------------
\begin{lemma}
The amortized time per-point to update the coreset tree $Q$ over a sequence of $n$ input batches is $O(kd)$.
\end{lemma}
%-------------------
\begin{proof}
For any level $\ell$ in $Q$, there are at most $r$ buckets. We generate a level $1$ bucket after receiving every $r$ input batches, and generate a level $2$ bucket after receiving every $r^2$ input batches, and so one. So with every $r^i$ input batches, a new bucket containing a level $i$ coreset is constructed. 
Using Theorem~\ref{theo:coreset build}, the time cost of merging $r$ buckets with total of $rm$ points into a new bucket at a higher level is $O(kdrm+\log^2(rm)+dk)$. 
So the amortized time for each point to update $Q$ is
\[ \begin{split} 
&\sum_{\ell=1}^{\left\lceil \log_r n \right\rceil}\frac{1}{r^{\ell}m}O(kdrm+\log^2(rm)+dk) \\
&=O\left(\frac{kdrm+\log^2(rm)+dk}{m(r-1)}\right) \\
&=O(kd)
\end{split}
\]
So the lemma is proved.
\end{proof}
%-------------------


%-------------------
\begin{lemma}
The amortized time per-point of Algorithm~\ref{algo:fkm-process} to return $k$ centers is $O(kdr)$.
\end{lemma}
%-------------------
\begin{proof}
To compute the final $k$ centers in each batch, we first generate two multisets: a set of buckets $b_Q$ from the coreset tree $Q$ and a bucket $b_{cache}$ from the $\cache$. As the merge degree is $r$, the number of buckets in $b_Q$ is at most $(r-1)$, so $b_Q$ contains at most $m(r-1)$ points. On the other hand, $b_{cache}$ contains $m$ points. To merge the multiset $b_Q$ and $b_{cache}$ into one bucket, using the Theorem~\ref{theo:coreset build}, the time cost is 
$O(kdmr+\log^2rm + kd)=O(kdmr)$. 
Note that we only insert new $\coreset$ in the cache once for every $r$ batches when the number of batches is divisible by $r$. So the amortized time to compute new $\coreset$ is $O(kdm)$.
Then we run the $\kmpp$ on the union set of $b_Q \cup b_{coreset}$, as the union set contains $O(mr)$ points, this spends time $O(kdmr)$. 
So the total time to return the $k$ centers is $O(kdmr)$ for each batch, as each batch contains $O(m)$ points, the amortized time complexity for each point is $O(kdr)$.
\end{proof}
%-------------------


%-------------------
\begin{lemma}
At timestep $n$, the amortized time per-point of $\skmpp$ to return $k$ centers is $O(kdr\log_r n)$.
\end{lemma}
%-------------------
\begin{proof}
At timestep $n$, the maximum level of coreset tree $Q$ is $\left\lfloor \log_r n \right\rfloor$ and each level has at most $r$ buckets. So in total there are $r\cdot \log_r n$ buckets in $Q$. 
We run the $\kmpp$ on the union of all the coresets in $Q$, which spends time $O(kdmr\log_r n)$. The amortized time per-point is $O(kdr\log_r n)$.
\end{proof}
%-------------------

%---------------------------------------------------------
\subsection{Comparison with \skmpp}
%---------------------------------------------------------
In \skmpp\cite{AMR+12}, coresets are constructed using the \kmpp algorithm. Suppose that a coreset size of $m$ was used (the paper says $m=200k$ is sufficient). The amortized cost of processing a batch of $m$ points using \skmpp is $O(dm^2)$, and the amortized per-item processing cost is $O(dm)$. In contrast, the cost of answering a query is $O(dm^2 \log(n/m) + dkm)$. If a query was answered after each input point (continuous maintenance), the cost of processing a query dominates the cost of processing a point. 


\remove{

Let $S$ be the set of all points observed till the current time.
%-------------------
\begin{lemma}
The centers returned by Algorithm Cluster-Centers is an $O(\log k)$ approximation to the optimal clustering of $S$.
\end{lemma}
%-------------------



\subsection{Faster Algorithm Using Coreset Caching}

(intuition idea, decompose each number into two part, and store the major part in the cache for future use.)

Before stepping into our algorithm to answer the query, we first introduce some notations and definitions.

\begin{definition}[Major and Minor]
\label{defn: major&minor}
Given a positive integer $n\in Z^+$, decompose $n$ into a sum of powers of $2$: 
\[
n = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_0} = \sum_{i=0}^j2^{\alpha_i}
\]
where $\alpha_j>\alpha_{j-1}>\cdots>\alpha_0\geq 0$. Note that for any positive integer, this decomposition is unique.
Define the function $minor(n) = 2^{\alpha_0}$ which is the least significant term in the decomposition expression.
We also define $major(n) = n - minor(n)$. When $n$ is the power of $2$, $major(n) = 0$. Otherwise, $major(n) = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_1}$.
\end{definition}

A partial sum of a series is the sum of a finite number of consecutive terms beginning with the first term. Based on the decomposition above, we have a series $S = \{2^{\alpha_j}, 2^{\alpha_{j-1}}, \ldots, 2^{\alpha_0}\}$, define the partial sum set of $n$ as the union of all the partial sums of series $S$, except number $n$ itself. The formal definition is as follows:

\begin{definition}[Partial Sum Set]
\label{defn: partial sum set}
$\forall n\in Z^+$, decompose $n$ into a sum of powers of $2$:
\[
n = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_0} = \sum_{i=0}^j2^{\alpha_i}
\]
where $\alpha_j>\alpha_{j-1}>\cdots>\alpha_0\geq 0$. 
Define set $S = \{2^{\alpha_j}, 2^{\alpha_{j-1}}, \ldots, 2^{\alpha_0}\}$ and $s_k$ represents sum of the first $k$ terms of set $S$ except $n$ itself, $s_k = \sum_{i=j-k}^j2^{\alpha_i}$, where $0 \leq k \leq j-1$. We define the partial sum set $partsum(n) = \bigcup_{k=0}^{j-1}s_k$. Note when $n$ is power of $2$, $partsum(n) = \emptyset$.
\end{definition}

The formal algorithm is as follows:
\newline

%----------------------
\begin{algorithm}
\caption{\sf At time $n$, answer a Query for cluster centers with caching}
\KwIn{Coreset Cache $L$}
\KwOut{$k$ cluster centers of stream $S_n$}
\BlankLine

$Q \leftarrow$ retrieve the multiset $Q_{minor(n)}$ in the updated coreset tree \;

\eIf {$major(n)=0$} {     
	$C_n \leftarrow Q$\;
} {
	$R \leftarrow$ retrieve coreset $major(n)$ from the cache $L$\;
	$C_n \leftarrow Merge(Q, R)$\;
}

Remove all coresets $\notin partsum(n)$ in $L$\;

Add $C_n$ to cache $L$\;

Return $k$-means++$(k, C_n)$\;
\end{algorithm}
%------------------------------------------------------------------------------------------------------

\textbf{Correctness}

\begin{lemma}
$\forall n\in Z^+$, $partsum(n)$ is always available in the cache $L$ at the beginning time of $n$.
\begin{proof}
We use mathematical induction in the proof.

$\textbf{Base case:}$ 
When $n=1$ and $2$, as these two numbers are powers of 2, so both of their $partsums$ are empty sets, we keep $1$ and $2$ in the cache.
At the beginning time of $n=3$, $partsum(3)=\{2\}$ and $2$ is in the cache.

$\textbf{Inductive step:}$
Suppose at beginning time of $n$, the $partsum(n)$ is in the cache. Based on the algorithm, at the beginning time of $(n+1)$, cache contains $partsum(n)$ and $n$. We claim $partsum(n+1) \subseteq partsum(n)\bigcup \{n\}$.

If $n$ is even, it is trivial as in binary format, the only bit changed from $n$ to $n+1$ is the last bit flips from $0$ to $1$, so $partsum(n+1) = partsum(n)\bigcup \{n\}$.

If $n$ is odd, there are two cases to consider.
When $n+1$ is power of $2$, the $partsum$ is empty set and $n+1$ is the only point in the cache at the end time of $n+1$. 
When $n+1$ is not power of 2, there must exist at least one $0$ bit in the binary format of $n$. $n+1$ will flip a streak of $1$ bits starting from the least significant bit, until it hits the first $0$ bit, which turns it into $1$. We refer the weight of the first $0$ bit in $n$ as $2^k$, so $n$ can be expressed as $n = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_m} + 2^{\alpha_{m-1}} + \cdots + 2^{\alpha_0}$, where the bit $\alpha_m$ is the least significant bit that greater than $k$, $\alpha_{m-1} < k < \alpha_{m}$. Correspondingly, $n+1 = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_m} + 2^k$. Comparing with $n$, $\alpha_j, \alpha_{j-1}, \cdots \alpha_m$ are unchanged, thus $partsum(n+1) \subset partsum(n)$. So in both cases, $partsum(n+1)$ is in the cache $L$ at the beginning time of $n+1$.
\end{proof}
\end{lemma}
Based on the lemma, when $n$ is not power of $2$, we have $major(n) \in partsum(n)$, so we can always retrieve coreset $major(n)$ from the cache. When $n$ is power of $2$, we directly retrieve the only coreset in the coreset tree. 

%------------------------------------------------------------------------------------------------------

\textbf{Time Complexity}
}
}


==> appx.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "kmeans"
%%% End:


==> binarymerge.tex <==
\subsection{Binary Coreset Tree}
Instead of using the naive aggregation method above, we design an algorithm reducing the time cost of aggregation with the expense of additional memory space. Our intuitive idea is to store the coresets aggregation result of previous rounds in the coreset cache $L$, then use the stored aggregation coresets to quickly calculate the new round coreset. We will show that by having very limited size of cache, we could achieve exactly one aggregation to generate the coreset, other than amortized $O(logn)$ in previous method.

\begin{algorithm}
\caption{{\sf Coreset Aggregation}}
\KwIn{time $n$; buffers $M_0, M_1, M_2, ... M_r$; coreset cache $L$}
\KwOut{coreset of current timeslot $C_n$}
\BlankLine

Decompose $n$ into the sum of powers of 2, $ n = 2^{a_1} + 2^{a_2} ... + 2^{a_j} $ with $a_1 > a_2 > ... > a_j$. Note this decomposition is unique\;
$Q \leftarrow$ retrieve $M_{a_j}$\;
$n' \leftarrow n - 2^{a_j} $\;

\eIf {$n'=0$} {     
	$C_n \leftarrow Q$\;
} {
	$C_{n'} \leftarrow$ retrieve from $L$\;
	$C_n \leftarrow Merge(Q, C'_n)$\;

}

\tcc{\qquad \qquad \qquad \qquad Add to cache}
\If {$n$ is even} {
	Add $C_n$ to $L$\;
}

\tcc{\qquad \qquad \qquad \qquad Delete from cache}
\If {$a_{j-1}-1=a_j$} {
	Remove $C_{n'}$ from $L$\;
}

\end{algorithm}


==> exp_stream.tex <==
%----------------
\begin{figure*}
  \centering
  \subfloat[\covtype]{
  \centering \includegraphics[width=0.23\textwidth]{expfigs/accuracy_num/covtype_cost_vs_num.pdf}
  }
  \subfloat[\power]{
  \centering \includegraphics[width=0.23\textwidth]{expfigs/accuracy_num/power_cost_vs_num.pdf}
  }
  \subfloat[\intrusion  (\seqkm not shown)]{
  \centering \includegraphics[width=0.23\textwidth]{expfigs/accuracy_num/intrusion_cost_vs_num.pdf}
  }
  \subfloat[\drift]{
  \centering \includegraphics[width=0.23\textwidth]{expfigs/accuracy_num/synthetic_cost_vs_num.pdf}
  }
\caption{\km cost vs. number of points. The number of clusters $k$ is $30$.}
\label{fig:cost-versus-stream}
\end{figure*}
%----------------

%----------------
\begin{figure*}
  \centering
  \subfloat[\covtype]{
  \centering \includegraphics[width=0.23\textwidth]{expfigs/totaltime_num/covtype_total_vs_num.pdf}
  }
  \subfloat[\power]{
  \centering \includegraphics[width=0.23\textwidth]{expfigs/totaltime_num/power_total_vs_num.pdf}
  }
  \subfloat[\intrusion]{
  \centering \includegraphics[width=0.23\textwidth]{expfigs/totaltime_num/intrusion_total_vs_num.pdf}
  }
  \subfloat[\drift]{
  \centering \includegraphics[width=0.23\textwidth]{expfigs/totaltime_num/synthetic_total_vs_num.pdf}
  }
  \caption{Average runtime per point (milliseconds) vs. number of points. The number of clusters $k$ is $30$.}
\label{fig:time-versus-stream}
\end{figure*}
%----------------

==> query.tex <==
%--------------------------------------------------------------------------------------------------
\section{Cache Size}
\label{sec:cache size}
%--------------------------------------------------------------------------------------------------

\subsection{prefix numbers}

Before stepping into our algorithm to answer the query, we first introduce some notations and definitions.

\begin{definition}[Major and Minor]
\label{defn: major&minor}
Given a positive integer $n\in Z^+$, decompose $n$ into a sum of powers of $2$: 
\[
n = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_0} = \sum_{i=0}^j2^{\alpha_i}
\]
where $\alpha_j>\alpha_{j-1}>\cdots>\alpha_0\geq 0$. Note that for any positive integer, this decomposition is unique.
Define the function $minor(n) = 2^{\alpha_0}$ which is the least significant term in the decomposition expression.
We also define $major(n) = n - minor(n)$. When $n$ is the power of $2$, $major(n) = 0$. Otherwise, $major(n) = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_1}$.
\end{definition}

A partial sum of a series is the sum of a finite number of consecutive terms beginning with the first term. Based on the decomposition above, we have a series $S = \{2^{\alpha_j}, 2^{\alpha_{j-1}}, \ldots, 2^{\alpha_0}\}$, define the partial sum set of $n$ as the union of all the partial sums of series $S$, except number $n$ itself. The formal definition is as follows:

\begin{definition}[Partial Sum Set]
\label{defn: partial sum set}
$\forall n\in Z^+$, decompose $n$ into a sum of powers of $2$:
\[
n = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_0} = \sum_{i=0}^j2^{\alpha_i}
\]
where $\alpha_j>\alpha_{j-1}>\cdots>\alpha_0\geq 0$. 
Define set $S = \{2^{\alpha_j}, 2^{\alpha_{j-1}}, \ldots, 2^{\alpha_0}\}$ and $s_k$ represents sum of the first $k$ terms of set $S$ except $n$ itself, $s_k = \sum_{i=j-k}^j2^{\alpha_i}$, where $0 \leq k \leq j-1$. We define the partial sum set $partsum(n) = \bigcup_{k=0}^{j-1}s_k$. Note when $n$ is power of $2$, $partsum(n) = \emptyset$.
\end{definition}


\begin{lemma}
$\forall n\in Z^+$, $partsum(n)$ is always available in the cache $L$ at the beginning time of $n$.
\begin{proof}
We use mathematical induction in the proof.

$\textbf{Base case:}$ 
When $n=1$ and $2$, as these two numbers are powers of 2, so both of their $partsums$ are empty sets, we keep $1$ and $2$ in the cache.
At the beginning time of $n=3$, $partsum(3)=\{2\}$ and $2$ is in the cache.

$\textbf{Inductive step:}$
Suppose at beginning time of $n$, the $partsum(n)$ is in the cache. Based on the algorithm, at the beginning time of $(n+1)$, cache contains $partsum(n)$ and $n$. We claim $partsum(n+1) \subseteq partsum(n)\bigcup \{n\}$.

If $n$ is even, it is trivial as in binary format, the only bit changed from $n$ to $n+1$ is the last bit flips from $0$ to $1$, so $partsum(n+1) = partsum(n)\bigcup \{n\}$.

If $n$ is odd, there are two cases to consider.
When $n+1$ is power of $2$, the $partsum$ is empty set and $n+1$ is the only element in the cache at the end time of $n+1$. 
When $n+1$ is not power of 2, there must exist at least one $0$ bit in the binary format of $n$. $n+1$ will flip a streak of $1$ bits starting from the least significant bit, until it hits the first $0$ bit, which turns it into $1$. We refer the weight of the first $0$ bit in $n$ as $2^k$, so $n$ can be expressed as $n = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_m} + 2^{\alpha_{m-1}} + \cdots + 2^{\alpha_0}$, where the bit $\alpha_m$ is the least significant bit that greater than $k$, $\alpha_{m-1} < k < \alpha_{m}$. Correspondingly, $n+1 = 2^{\alpha_j}+2^{\alpha_{j-1}}+ \cdots + 2^{\alpha_m} + 2^k$. Comparing with $n$, $\alpha_j, \alpha_{j-1}, \cdots \alpha_m$ are unchanged, thus $partsum(n+1) \subset partsum(n)$. So in both cases, $partsum(n+1)$ is in the cache $L$ at the beginning time of $n+1$.
\end{proof}
\end{lemma}



==> related.tex <==
\subsection{Related Work}
\label{sec:related}
%------------------------------------------
The literature on $k$-means clustering has a long and rich history.  In the
\emph{batch} setting (all the input is available at the start of the
computation), Lloyd's algorithm~\cite{Lloyd82}, also known as \km algorithm, has
been used for \km clustering for decades and is a simple iterative procedure
that is widely used in practice. However, it does not have a good (theoretical)
guarantee on the quality of the clusters. \kmpp~\cite{AV07} suggests a new
seeding procedure to determine the starting configuration for Lloyd's algorithm
with a provable guarantee on the quality of the clusters with respect to the
optimal solution. Bahmani et~al.~propose a parallel algorithm
\kmII~\cite{BMV+12} that reduces the number of iterations in the initialization
phase of \kmpp algorithm.

%Streaming
The earliest streaming clustering method appears in \cite{MacQueen67} , which
simply applies Lloyd's algorithm for every new point received. Because it is
fast and easy to implement, this simple algorithm has been widely used in
practice (e.g., Apache Spark mllib~\cite{MBY+15}). However, it cannot provide
any good clustering quality guarantees~\cite{KMN+04}. In \cite{AD14}, Ackerman
and Dasgupta state the limitations of sequential clustering and study the case
where extra clusters are allowed to improve the quality.  In the past $20$
years, with a rapid increase in the size of datasets and the rise of database
technology, many modern clustering methods for data stream operate on the
assumption that it is impossible to fit the whole data in memory.
\textit{BIRCH}~\cite{ZRL96} is one of the earliest and well-known clustering
method for data stream. The \textit{BIRCH} algorithm builds and maintains a
special data structure called \textit{CF Tree}, and returns cluster centers by
applying agglomerative hierarchical clustering algorithm on all the leaf nodes
in the CF Tree. As another well-known stream clustering algorithm,
\textit{CluStream}\cite{AHW+03} clusters the data stream based on a new concept
of \textit{microcluster}, which summarizes a set of statistics of the instances
from the stream. The algorithm returns the cluster centers by applying a
weighted \km algorithm on the microclusters. \cite{GMM+03} present a
hierarchical divide-and-conquer method called \textit{STREAMLS}. Their method is
based on repeated application of a bicriteria approximation algorithm for
clustering. A similar streaming based on the \kmpp algorithm is presented
in~\cite{AJM09}. However, these methods have a high cost of query processing,
and is not suitable for continuous maintenance of clusters in a stream. In
particular, each time the set of cluster centers has to be returned, it requires
merging multiple data structures, followed by an extraction of the centers,
which is expensive. We will provide a more detailed comparison with our work in
later sections.

%Coreset
Recently, there has been interest in generating a compact summary, known as a
\emph{coreset}, of the original data~\cite{AHV04}.  A coreset is a much smaller
set of points than the original that approximately maintains the properties of
the original point with respect to a certain problem. For \km, Har-Peled first
shows the existence of the coreset with size $O(k\epsilon^d \log n)$
in~\cite{HM04}, where $n$ is the total number of points. \cite{HM04} also put
forward a stream clustering algorithm using coreset by applying the
merge-and-reduce technique, which is based on the Bentley-Saxe
decomposition~\cite{BS80}. In~\cite{HK07}, Har-Peled reduces the size of the
coreset to $O(k^3/\epsilon^{d+1})$. More recently, Feldman\cite{FL11} provides a
coreset with size $O(\frac{kd}{\epsilon^6})$.

\skmpp~\cite{AMR+12} is a streaming $k$-means clustering algorithm that is built
on the \kmpp algorithm to generate coreset. Our work improves on \skmpp in terms
of speed. There are many other stream clustering algorithms; we refer interested
readers to~\cite{AMR+12} and the references therein.

%  still a lot of stream clustering algorithms, but will not
% list all of them here.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "kmeans"
%%% End:

